A Game-Theoretic Framework for AI Governance

As a transformative general-purpose technology, AI has empowered various industries and will continue to shape our lives through ubiquitous applications. Despite the enormous benefits from wide-spread AI deployment, it is crucial to address associated downside risks and therefore ensure AI advances are safe, fair, responsible, and aligned with human values. To do so, we need to establish effective AI governance. In this work, we show that the strategic interaction between the regulatory agencies and AI firms has an intrinsic structure reminiscent of a Stackelberg game, which motivates us to propose a game-theoretic modeling framework for AI governance. In particular, we formulate such interaction as a Stackelberg game composed of a leader and a follower, which captures the underlying game structure compared to its simultaneous play counterparts. Furthermore, the choice of the leader naturally gives rise to two settings. And we demonstrate that our proposed model can serves as a unified AI governance framework from two aspects: firstly we can map one setting to the AI governance of civil domains and the other to the safety-critical and military domains, secondly, the two settings of governance could be chosen contingent on the capability of the intelligent systems. To the best of our knowledge, this work is the first to use game theory for analyzing and structuring AI governance. We also discuss promising directions and hope this can help stimulate research interest in this interdisciplinary area. On a high, we hope this work would contribute to develop a new paradigm for technology policy: the quantitative and AI-driven methods for the technology policy field, which holds significant promise for overcoming many shortcomings of existing qualitative approaches.

==> case.tex <==
No one-fit-all solution. The answer should be industry-specific. 

In this section, we instantiate the Stakelberg game framework proposed in the previous section. The key is carefully construct the objective functions for AI corporations player and regulatory agencies player separately. Based on this, we can solve the game as a bi-level optimization problem. We end this section by analyzing the equilibrium properties and implications. 

\subsection{Build Return and Risk Models }
[Note that building these models on a firm level could leverage insights and research from the evaluation group or other groups with relevant expertise.] 
As part of the market economy, AI corporations and organizations would seek to reap returns AI. 

The AI corporations/institutions seeks to maximize the return from AI innovation and application and their objective function can be modeled as follows: [to be added]. 

%\begin{align}\label{return_auto}
   
%\end{align}


The loss function of the AI regulatory agencies is defined as [to be added]. 

%\begin{align}\label{loss_auto}
    
%\end{align}



\subsection{Instantiate Stackelberg Framework}
With the objective functions proposed in the preceding section, it is straightforward to instantiate the Stackelberg framework described in section 3. 

\subsection{Algorithms and Equilibrium Analysis}


\subsection{Implications}


